kNN-Embed: Locally Smoothed Embedding Mixtures For Multi-interest Candidate Retrieval

Candidate retrieval is the first stage in recommendation systems, where a light-weight system is used to retrieve potentially relevant items for an input user. These candidate items are then ranked and pruned in later stages of recommender systems using a more complex ranking model. As the top of the recommendation funnel, it is important to retrieve a high-recall candidate set to feed into downstream ranking models. A common approach is to leverage approximate nearest neighbor (ANN) search from a single dense query embedding; however, this approach this can yield a low-diversity result set with many near duplicates. As users often have multiple interests, candidate retrieval should ideally return a diverse set of candidates reflective of the user's multiple interests. To this end, we introduce kNN-Embed, a general approach to improving diversity in dense ANN-based retrieval. kNN-Embed represents each user as a smoothed mixture over learned item clusters that represent distinct "interests" of the user. By querying each of a user's mixture component in proportion to their mixture weights, we retrieve a high-diversity set of candidates reflecting elements from each of a user's interests. We experimentally compare kNN-Embed to standard ANN candidate retrieval, and show significant improvements in overall recall and improved diversity across three datasets. Accompanying this work, we open source a large Twitter follow-graph dataset (https://huggingface.co/datasets/Twitter/TwitterFollowGraph), to spur further research in graph-mining and representation learning for recommender systems.

==> 03preliminaries.tex <==


\section{Preliminaries}\label{sec:preliminaries}
Let $\mathcal{U} = \{u_1, u_2, \ldots u_n\}$ be the set of source entities (i.e., users in a recommender system) and $\mathcal{I} = \{i_1, i_2, \ldots i_m\}$ be the set of target entities (i.e., items in a recommender system). Let $\mathcal{G}$ constitute a bipartite graph representing the engagements between users ($\mathcal{U}$) and items ($\mathcal{I}$). For each user and item, we define a ``relevance'' variable in $\{0, 1\}$ indicating an item's relevance to a particular user. An item is considered relevant to a particular user if a user, presented with an item, will engage with said item. Based on the engagements in $\mathcal{G}$, each user, $u_j$, is associated with  a $d$-dimensional embedding vector $\mathbf{u_j} \in \mathbb{R}^d$; similarly each target item $i_k$ is associated with an embedding vector $\mathbf{i_k} \in \mathbb{R}^d$. We call these  the \emph{unimodal} embeddings, and assume that they model user-item relevance $p(\textrm{relevance} | u_j, i_k) = f(\mathbf{u_j}, \mathbf{i_k})$ for a suitable function $f$.

Given the input user-item engagement graph, our goal is to learn mixtures of embeddings representations of users that better capture the multiple interests of a user as evidenced by higher recall in a candidate retrieval task.






